Macroscopic Thermodynamic Reversibility in Quantum Many-Body Systems

The resource theory of thermal operations, an established model for small-scale thermodynamics, provides an extension of equilibrium thermodynamics to nonequilibrium situations. On a lattice of any dimension with any translation-invariant local Hamiltonian, we identify a large set of translation-invariant states that can be reversibly converted to and from the thermal state with thermal operations and a small amount of coherence. These are the spatially ergodic states, i.e., states that have sharp statistics for any translation-invariant observable, and mixtures of such states with the same thermodynamic potential. As an intermediate result, we show for a general state that if the min- and the max-relative entropy to the thermal state coincide approximately, this implies the approximately reversible interconvertibility to and from the thermal state with thermal operations and a small source of coherence. Our results provide a strong link between the abstract resource theory of thermodynamics and more realistic physical systems, as we achieve a robust and operational characterization of the emergence of a thermodynamic potential in translation-invariant lattice systems.

==> bibolamazi_dup_aliases.tex <==
%
% NOTE: THIS FILE WAS AUTOMATICALLY GENERATED BY bibolamazi SCRIPT!
%       ANY CHANGES WILL BE LOST!
%
% File automatically generated by bibolamazi's `duplicates` filter.
%
% You should include this file in your main LaTeX file with the command
%
%   \input{bibolamazi_dup_aliases.tex}
%
% in your document preamble.
%



%
% The following will define the command \bibalias{<alias>}{<source>}, which will make
% the command \cite[..]{<alias>} the same as doing \cite[..]{<source>}.
%
% This code has been copied and adapted from
%    http://tex.stackexchange.com/questions/37233/
%

\makeatletter
% \bibalias{<alias>}{<source>} makes \cite{<alias>} equivalent to \cite{<source>}
\newcommand\bibalias[2]{%
  \@namedef{bibali@#1}{#2}%
}


% Code taken from from etextools.sty, apparently originally borrowed from environ.sty
\newcommand\biba@deblank[1]{\romannumeral\biba@deblank@#1/ /} % dark magic. stay away
\long\def\biba@deblank@#1 /{\biba@deblank@i#1/}
\long\def\biba@deblank@i#1/#2{\z@#1}


\newtoks\biba@toks
\let\bibalias@oldcite\cite
\def\cite{%
  \@ifnextchar[{%
    \biba@cite@optarg%
  }{%
    \biba@cite{}%
  }%
}
\newcommand\biba@cite@optarg[2][]{%
  \biba@cite{[#1]}{#2}%
}
\newcommand\biba@cite[2]{%
  \biba@toks{\bibalias@oldcite#1}%
  \def\biba@comma{}%
  \def\biba@all{}%
  \def\biba@argkeys{}%
  \@for\biba@one@:=#2\do{%
    \edef\biba@one{\expandafter\@firstofone\biba@one@\@empty}%
    \edef\biba@one{\expandafter\biba@deblank\expandafter{\biba@one}}% remove whitespace
    \edef\biba@argkeys{\biba@argkeys\biba@comma\biba@one}%
    \@ifundefined{bibali@\biba@one}{%
      \edef\biba@all{\biba@all\biba@comma\biba@one}%
    }{%
      \PackageInfo{bibalias}{%
        Replacing citation `\biba@one' with `\@nameuse{bibali@\biba@one}'
      }%
      \edef\biba@all{\biba@all\biba@comma\@nameuse{bibali@\biba@one}}%
    }%
    \def\biba@comma{,}%
  }%
  %
  % However, still write in the .aux file a dummy \citation{...} command, so that
  % filters.util.auxfile will still catch those used citations
  %
  \immediate\write\@auxout{\noexpand\bgroup\noexpand\renewcommand\noexpand\citation[1]{}\noexpand\citation{\biba@argkeys}\noexpand\egroup}%
  %
  % Now, produce the \cite command with the original keys instead of the aliases
  %
  \edef\biba@tmp{\the\biba@toks{\biba@all}}%
  \biba@tmp%
}
\makeatother


%
% Now, declare all the alias keys.
%

\bibalias{Bjelakovic2003arXiv_compression}{Bjelakovic2005QIP_compression}
\bibalias{Chitambar2018arXiv_resource}{Chitambar2019RMP_resource}
\bibalias{Chubb2017arXiv_beyond}{Chubb2018Qu_beyond}
\bibalias{Gour2017arXiv_entropic}{Gour2018NatComm_entropic}
\bibalias{HindsMingo2018arXiv_multiple}{HindsMingo2018_multiple}
\bibalias{Popescu2018arXiv_applications}{Popescu2018PTRSA_applications}
\bibalias{Weilenmann2018arXiv_smooth}{Weilenmann2018_smooth}



